Large Language Models for Multilingual Code Intelligence: A Survey

Large language models have transformed AI-assisted software engineering, but current research remains biased toward high-resource languages such as Python, with weaker performance in languages like Rust and OCaml. Since real-world systems are inherently polyglot, robust multilingual code intelligence is crucial. This survey focuses on two key tasks: multilingual code generation from shared natural-language requirements, and multilingual code translation that preserves semantics across languages. It reviews representative methods, benchmarks, and evaluation metrics, and highlights challenges and opportunities for trustworthy cross-language generalization.

==> Figure/Code-gen-and-trans.tex <==
\begin{figure}[t]
\vspace{-2.5pt}
    \centering
    \includegraphics[width=0.75\textwidth]{images/code-gen-trans.png}
    \setlength{\abovecaptionskip}{5pt}
    \setlength{\belowcaptionskip}{-15pt}
    \caption{Two Core Tasks: Multilingual Code Generation Vs.  Translation}
    \label{fig:cgat}
\end{figure}

==> Figure/PL-frequency.tex <==
\begin{figure}[t]
\vspace{-5pt}
    \centering
    \includegraphics[width=0.75\textwidth]{images/pl_frequency.png}
    \setlength{\abovecaptionskip}{-0pt}
    \setlength{\belowcaptionskip}{-10pt}
    \caption{Programming Language Frequency in Surveyed Research}
    \label{fig:pl_frequency}
\end{figure}

==> Figure/Statistics.tex <==
\begin{figure}[t]
\vspace{-5pt}
    \centering
    \includegraphics[width=1.0\textwidth]{images/statistics.png}
    \setlength{\abovecaptionskip}{-0pt}
    \setlength{\belowcaptionskip}{-10pt}
    \caption{Statistics}
    \label{fig:statistics}
\end{figure}

==> Table/Comparison-of-two-tasks.tex <==
\begin{table}[t]
    \footnotesize
    \centering
    \setstretch{1.15}
    \setlength{\tabcolsep}{2pt}
    \setlength{\abovecaptionskip}{2.5pt}
    \setlength{\belowcaptionskip}{-2.5pt}
    \caption{Comparison between Multilingual Code Generation and Translation}
    \label{tab:task_comparison}
    \resizebox{1\linewidth}{!}{%
    \begin{tabular}{cll}
        \hline
        \textbf{Feature} & \textbf{Code Generation} & \textbf{Code Translation} \\ \hline
        \textbf{Operational\,Goal} & Create a program to fit specific environments. & Move an existing program to a target environment. \\ 
        \textbf{Input\,Source} & Abstract intent ($NL$). & Concrete execution logic ($PL_{source}$). \\ 
        \textbf{Key\,Constraint} & Environmental suitability \& syntax. & Semantic invariance \& functional equivalence. \\ 
        \textbf{Analogy} & Building a new house from a blueprint. & Relocating a house to a new foundation. \\ \hline
    \end{tabular}}
    \vspace{-7.5pt}
\end{table}

==> Table/Table0.tex <==
\begin{table}[ht]
\centering
\setstretch{1.35}
\setlength{\tabcolsep}{5.5pt}
\setlength{\abovecaptionskip}{2.5pt}
\setlength{\belowcaptionskip}{-2.5pt}
\caption{Taxonomy of Research on LLMs for Code Generation and Translation.}
\label{tab:taxonomy}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llcclc}
\hline
\textbf{\small Category} & \textbf{\small Approach} & \textbf{\small Year} & \textbf{\small \begin{tabular}[c]{@{}l@{}}Programming\\Language\end{tabular}} & \textbf{\small \begin{tabular}[c]{@{}l@{}}Static Large Language\\Models\end{tabular}} & \textbf{\small \begin{tabular}[c]{@{}l@{}}Static Analyzer\\Integration\end{tabular}} 
\vspace{5pt}
\\ 
\hline
\multirow{16}{*}{\small\textbf{\begin{tabular}[c]{@{}l@{}}LLM as\\a static\\analyzer\end{tabular}}}  & SkipAnalyzer~\cite{mohajer2023skipanalyzer} & 2025 & Java & GPT-3.5, GPT-4 & -- \\
 & Fang et al.~\cite{fang2024large} & 2024 & \begin{tabular}[c]{@{}l@{}}C, JavaScript,\\Python\end{tabular} & \begin{tabular}[c]{@{}l@{}}GPT-3.5, GPT-4,\\LLaMA-2, Code-LLaMA\end{tabular} & -- \\
 & Ignatyev et al.~\cite{ignatyev2024large} & 2024 & C++, C\#, Java & CodeLlama-34B-v2 & -- \\
 & E\&V~\cite{hao2023v} & 2024 & Pseudo Code& GPT-4 & -- \\
 & Mohajer et al.~\cite{mohajer2024effectiveness} & 2024 & C/C++ & GPT-3.5, GPT-4 & -- \\
 & CORE~\cite{xie2025core} & 2024 & \begin{tabular}[c]{@{}l@{}}C/C++, Java,\\Python \end{tabular}  & \begin{tabular}[c]{@{}l@{}}Claude, DeepSeek,\\Qwen3, GPT \end{tabular} & -- \\
 & Çetin et al.~\cite{ccetin2024empirical} & 2024 & PHP & \begin{tabular}[c]{@{}l@{}}GPT-3.5, GPT-4,\\Claude, Gemini1, Llama-2\end{tabular} & -- \\
 & LLMDFA~\cite{wang2024llmdfa} & 2025 & C/C++ & \begin{tabular}[c]{@{}l@{}}GPT-3.5, GPT-4,\\Claude, Gemini1\end{tabular}  & -- \\
 & Zuraiqi et al.~\cite{al2025evaluation} & 2025 & C/C++ & Unknown & -- \\
 & GNIECIAK et al.~\cite{gnieciak2025large} & 2025 & C\# & GPT-4.1, DeepSeek V3 & -- \\
 & Su et al.~\cite{su2025code} & 2025 & C, Java & \begin{tabular}[c]{@{}l@{}}GPT-4o, Gemini,\\CodeLLaMA\end{tabular}  & -- \\
 & Abtahi et al.~\cite{abtahi2025augmenting} & 2025 & Java, JavaScript & GPT-3.5, GPT-4o & --
 \vspace{5pt}
\\ 
\hline
\multirow{7}{*}{\textbf{\small\begin{tabular}[c]{@{}l@{}}Filtering\\from\\existing\\analyzers\end{tabular}}} & Li et al.~\cite{li2023assisting} & 2023 & C/C++ & GPT-3.5, GPT-4 & UBITect \\
 & LLM4SA~\cite{wen2024automatically} & 2024 & C/C++ & GPT-3.5, LLaMA & \begin{tabular}[c]{@{}l@{}}CSA, Infer\\Cppcheck\end{tabular} \\
 & SAST~\cite{apostolidis2025ai} & 2025 & C/C++ & CodeBERT (fine-tuned) & Cppcheck \\
 & LLift~\cite{li2024enhancing} & 2025 & C/C++ & GPT-3.5, GPT-4 & UBITect \\
 & Jaoua et al.~\cite{jaoua2025combining} & 2025 & Java & Llama3-70B & PMD, Checkstyle \\
 & BinLLM~\cite{pan2025large} & 2025 & C/C++ & GPT-4o & Bingo  
 \vspace{5pt}
\\ 
\hline
\multirow{6}{*}{\textbf{\small\begin{tabular}[c]{@{}l@{}}Neuro-\\symbolic\\static\\analyzers\end{tabular}}} & CFStra~\cite{su2024cfstra} & 2024 & C/C++ & GPT-3.5 & CPAChecker \\
 & AutoSpec~\cite{wen2024enchanting} & 2025 & C/C++ & \begin{tabular}[c]{@{}l@{}}GPT-3.5, GPT-4,\\Llama-2\end{tabular} & Frama-C \\
 & Knighter~\cite{yang2025knighter} & 2025 & C/C++ & \begin{tabular}[c]{@{}l@{}}GPT-4o, DeepSeek-R1,\\Gemini-2-flash\end{tabular} & LLM Checkers \\
 & PropertyGPT~\cite{liu2025propertygpt} & 2025 & Solidity & GPT-4 & KSolidity \vspace{5pt}
\\ 
\hline
\end{tabular}%
}
\vspace{-10pt}
\end{table}

==> Table/Table3.tex <==
\begin{table}[t]
\centering
\setstretch{1.05}
\setlength{\tabcolsep}{3.5pt}
\setlength{\abovecaptionskip}{2.5pt}
\setlength{\belowcaptionskip}{-2.5pt}
% \caption{Taxonomy of LLMs for Multilingual Code Generation and Translation. \color{red}{(please kindly add ~\cite{wang2025evoc2rust} and ~\cite{aljagthami2025evaluating} into the table)}}
\caption{Taxonomy of LLMs for Multilingual Code Generation and Translation.}
\label{tab:test}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llcclc}
\hline
\textbf{\small Category} & \textbf{\small Approach} & \textbf{\small Year} & \textbf{\small \begin{tabular}[c]{@{}l@{}}Programming\\Languages\end{tabular}} & \textbf{\small \begin{tabular}[c]{@{}l@{}}Tasks\end{tabular}} 
\vspace{5pt}
\\ 
\hline
\multirow{20}{*}{\small\textbf{\begin{tabular}[c]{@{}l@{}}Multi-task\end{tabular}}}  
 & McEval~\cite{chai2024mceval} & 2024 & \begin{tabular}[c]{@{}l@{}}AWK, C, C\#, C++, Clojure, CoffeeScript, Common Lisp, Dart, \\Elixir, Emacs Lisp, Erlang, F\#, Fortran, Groovy, Go, HTML, \\Haskell, JSON, Java, JavaScript, Julia, Kotlin, Lua, Markdown,\\PHP, Pascal, Perl, PowerShell, Python, R, Racket, Ruby, \\Rust, Scala, Scheme, Shell, Swift, Tcl, TypeScript, \\VimScript, Visual Basic\end{tabular} & \begin{tabular}[c]{@{}l@{}}Code Generation, \\Code Completion, \\Code Explanation\end{tabular}\\
& XCODEEVAL~\cite{khan2024xcodeeval} & 2024 &\begin{tabular}[c]{@{}l@{}}C, C\#, C++, D, Go, Haskell, Java, JavaScript, Kotlin, \\OCaml, PHP, Pascal, Perl, Python, Ruby, Rust, Scala\end{tabular} & \begin{tabular}[c]{@{}l@{}}Code Generation, \\Code Translation, \\Code Retrieval\end{tabular} \\
& CodeNet~\cite{puri2021codenet} & 2021 & C++, Python, Java, C, Ruby, C\# & \begin{tabular}[c]{@{}l@{}}Code Similarity, \\Code Translation, \\Code Classification, \\Code Performance Improvement, \\Code Repair, \\Clone Detection, \\Code Search, \\Code Completion, \\Error Prediction\end{tabular} \\
& CodeXGLUE~\cite{lu2021codexglue} & 2021 & Java, C++, C, Python, PHP, JavaScript, Ruby, Go, C\# & \begin{tabular}[c]{@{}l@{}}Code Generation, \\Code Translation, \\Code Completion, \\Code Repair, \\Clone Detection, \\Defect Detection, \\Code Summarization, \\Code Search\end{tabular} \\
 \vspace{5pt}
\\ 
\hline
\multirow{4}{*}{\textbf{\small\begin{tabular}[c]{@{}l@{}}Code Generation\end{tabular}}} 
& mHumanEval~\cite{raihan2025mhumaneval} & 2025 & \begin{tabular}[c]{@{}l@{}}Python, Java, C++, JavaScript, Ruby, PHP, Go, Rust, Fortran,\\C\#, Lua, TypeScript, Scala, Kotlin, R, Dart, Swift, Perl, SQL,\\Haskell, OCaml, Shell, MATLAB, Visual Basic, COBOL\end{tabular} & Code Generation \\
& HumanEval-XL~\cite{peng2024humaneval} & 2024 & \begin{tabular}[c]{@{}l@{}}Python, Java, JavaScript, C\#, Go, Kotlin, \\PHP, Perl, Ruby, Swift, Scala, TypeScript\end{tabular} & Code Generation \\
 & MBPP~\cite{austin2021program} & 2021 & Python & \begin{tabular}[c]{@{}l@{}}Code Generation\end{tabular}
\\ 
\hline
\multirow{15}{*}{\textbf{\small\begin{tabular}[c]{@{}l@{}}Code Translation\end{tabular}}} 
& PSEUDOEVAL~\cite{wu2025isolating} & 2025 & Python, C++, Rust & Code Generation \\
& RepoTransBench~\cite{wang2024repotransbench} & 2024 & \begin{tabular}[c]{@{}l@{}}C, C++, C\#, Java, JavaScript, Matlab, Python, Go, Rust\end{tabular} & Code Translation \\
& G-TransEval~\cite{jiao2023evaluation} & 2023 & C++, Java, C\#, Python, JavaScript & Code Translation \\
& Codetransocean~\cite{yan2023codetransocean} & 2023 & \begin{tabular}[c]{@{}l@{}}Python, C, C++, C\#, Java, Go, PHP, Visual Basic, Ada, Swift,\\Arturo, AutoHotKey, AWK, BBC Basic, Clojure, Common Lisp,\\Delphi, Elixir, Erlang, Factor, Forth, Fortran, F\#, Groovy, Haskell, \\Icon, Julia, Mathematica, Lua, MATLAB, Nim, OCaml, Pascal,\\ Perl, PowerShell, J, R, Racket, REXX, Ruby, Rust, D, Scala, \\Tcl, COBOL\end{tabular} & Code Translation \\
& XLCoST~\cite{zhu2022xlcost} & 2022 & C++, Java, Python, C\#, JavaScript, PHP, C & \begin{tabular}[c]{@{}c@{}}Code Generation, \\Code Translation, \\Code Summarization, \\Code Search, \end{tabular} 
\\
\\ 
\hline
\end{tabular}%
}
\vspace{-10pt}
\end{table}

==> Tex/5-Discussion.tex <==
Despite significant progress, multilingual code intelligence remains constrained by a set of fundamental challenges that extend beyond model scale or prompt design. These challenges are structural in nature—rooted in data availability, evaluation practices, and the intrinsic diversity of programming paradigms. At the same time, they point to promising research opportunities for advancing robust and trustworthy polyglot software intelligence.


\smallskip
\textbf{C1: Fragmented Tasks and Unified Multilingual Capability.}
Multilingual code intelligence encompasses a wide spectrum of tasks, including code generation, translation, completion, repair, search, summarization, clone detection, and explanation, as shown in Fig.~\ref{fig:task_distributio}. 
While this diversity reflects the broad scope of real-world software engineering, current research typically studies these tasks in isolation, using task-specific datasets and evaluation protocols.
This fragmentation poses a fundamental challenge: models must handle many heterogeneous tasks while simultaneously maintaining robust multilingual capability. Strong performance on a single task or language does not necessarily translate to consistent performance across tasks, languages, and software contexts, making it difficult to assess true polyglot intelligence.

\vspace{-0.5ex}
\begin{tcolorbox}[size=title, opacityfill=0.1]
	\textbf{O1: General-Purpose Multilingual Code Intelligence.} An important research direction is the development of general-purpose multilingual models and unified benchmarks that jointly evaluate multiple code intelligence tasks. Approaches based on shared semantic representations, multi-task learning, and language-agnostic abstractions may enable models to achieve consistently strong performance across tasks and programming languages, moving toward robust and scalable multilingual code intelligence.
\end{tcolorbox}


\smallskip
\textbf{C2: Monolingual Bias and Data Imbalance.}
A core challenge is the pervasive monolingual bias in current research~\cite{joel2024survey}. This bias arises from skewed training corpora and evaluation benchmarks, which disproportionately favor mainstream languages.
As illustrated in Fig~\ref{fig:pl_frequency}, the distribution of programming languages in current research landscape is highly skewed; while mainstream languages like Python, C++, and Java dominate the frequency (with 13, 12, and 11 occurrences respectively), a vast majority of languages—such as Erlang, Haskell, and COBOL—occupy a ``long tail'' with minimal representation.
This imbalance limits cross-language generalization and leads to misleading performance gains that do not translate to real-world polyglot systems.

\vspace{-0.5ex}
\begin{tcolorbox}[size=title, opacityfill=0.1]
	\textbf{O2: Multilingual Alignment across Different Languages.} Future work should prioritize multilingual alignment by treating low-resource and paradigm-diverse languages as first-class targets. Approaches based on language-agnostic intermediate representations, semantic abstractions, and data-efficient learning offer a path toward reducing dependence on high-resource languages and achieving more balanced polyglot competence.
\end{tcolorbox}



\smallskip
\textbf{C3: Code Trustworthiness and Functional Correctness.}
Most evaluation frameworks emphasize functional execution, yet correctness alone is insufficient for trustworthy software. Multilingual code generation and translation often introduce subtle vulnerabilities, performance regressions, or maintainability issues that evade test-based evaluation.
This gap is particularly problematic in system-level and safety-critical domains, where trustworthiness is paramount.

\vspace{-0.5ex}
\begin{tcolorbox}[size=title, opacityfill=0.1]
	\textbf{O3: Integrating Verification, Safety, and Quality Signals.} A promising direction is the integration of LLMs with static analyzers, security checkers, and formal verification tools to enforce non-functional guarantees and functional correctness. Moving toward provable or constraint-aware code generation can significantly enhance trust in multilingual systems.
\end{tcolorbox}



%This data sparsity directly hinders the model's ability to learn robust representations for underrepresented languages. Furthermore, most current frameworks operate at a snippet-level, often failing to capture the complex, cross-file dependencies and modular architectures inherent in real-world software engineering. Multilingual code translation also frequently suffers from a lack of idiomaticity, where models prioritize literal syntactical alignment over the unique paradigms and safety guarantees of the target language—such as ownership in Rust or specific concurrency patterns in Go. Current evaluation metrics also remain overly reliant on surface-level functional execution, largely neglecting critical non-functional requirements like security, computational efficiency, and long-term maintainability.

%\textbf{Opportunity}. Looking forward, the field must evolve from simple sequence-to-sequence mapping toward deep logical understanding and repository-wide reasoning. A promising frontier lies in the integration of LLMs with formal verification tools and automated solvers, enabling the generation of code that is not only functional but also provably correct against formal specifications. By utilizing intermediate representations or "chain-of-thought" reasoning in pseudocode, future models can better decouple abstract logic from language-specific syntax, thereby narrowing the performance gap for underrepresented languages. Ultimately, the transition from passive code completion to autonomous, agentic systems capable of self-debugging and architectural planning will redefine the boundaries of multilingual software intelligence.
